RADIO-ViPE: Online Tightly Coupled Multi-Modal Fusion for Open-Vocabulary Semantic SLAM in Dynamic Environments

We present RADIO-ViPE (Reduce All Domains Into One -- Video Pose Engine), an online semantic SLAM system that enables geometry-aware open-vocabulary grounding, associating arbitrary natural language queries with localized 3D regions and objects in dynamic environments. Unlike existing approaches that require calibrated, posed RGB-D input, RADIO-ViPE operates directly on raw monocular RGB video streams, requiring no prior camera intrinsics, depth sensors, or pose initialization. The system tightly couples multi-modal embeddings -- spanning vision and language -- derived from agglomerative foundation models (e.g., RADIO) with geometric scene information. This coupling takes place in initialization, optimization and factor graph connections to improve the consistency of the map from multiple modalities. The optimization is wrapped within adaptive robust kernels, designed to handle both actively moving objects and agent-displaced scene elements (e.g., furniture rearranged during ego-centric session). Experiments demonstrate that RADIO-ViPE achieves state-of-the-art results on the dynamic TUM-RGBD benchmark while maintaining competitive performance against offline open-vocabulary methods that rely on calibrated data and static scene assumptions. RADIO-ViPE bridges a critical gap in real-world deployment, enabling robust open-vocabulary semantic grounding for autonomous robotics and unconstrained in-the-wild video streams. Project page: https://be2rlab.github.io/radio_vipe

==> tables/dynamic.tex <==
\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        \textbf{Method} & \textbf{RMSE (cm)} & \textbf{Tracking Lost} \\
        \midrule
        SamSLAM~\cite{SamSLAM} & 8.9 & 12\% \\
        ORB-SLAM3~\cite{ORB-SLAM3} & 14.2 & 38\% \\
        SplaTAM~\cite{splatam} & 6.7 & 8\% \\
        \textbf{Ours} & \textbf{5.1} & \textbf{4\%} \\
        \bottomrule
    \end{tabular}
    \caption{Dynamic Scene Performance (TUM-RGBD)}
    \label{tab:dynamic}
\end{table}

==> tables/grounding.tex <==
\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        \textbf{Method} & \textbf{Success Rate} & \textbf{mIoU} \\
        \midrule
        OpenScene~\cite{openscene} & 72\% & 63.2 \\
        ConceptGraphs~\cite{concept-graphs} & 81\% & 68.7 \\
        BBQ~\cite{bbq} & 78\% & 66.1 \\
        \textbf{Ours} & \textbf{89\%} & \textbf{73.5} \\
        \bottomrule
    \end{tabular}
    \caption{Language Grounding Performance}
    \label{tab:grounding}
\end{table}

==> tables/semantics-aria.tex <==
\begin{table}[ht]
    \centering
    \small
    % \setlength{\tabcolsep}{1.5pt} % Reduce column separation
    \caption{Semantic Segmentation Evaluation on Aria}
    \begin{tabular}{lccc}
        \toprule
        Scene & mIoU & fmIoU & mAcc \\
        \midrule
        seq102  & 1.9 & 5.8 & 4.6 \\
        seq134  & 1.8 & 7.0 & 4.7 \\
        seq133  & 1.1 & 5.0 & 4.1 \\
        \hline
        head & 5.1 & 7.1 & 12.5 \\
        common & 0.1 & 0.1 & 0.8 \\
        tail & 0.0 & 0.0 & 0.2 \\
        \midrule
        overall & 1.7 & 6.5 & 4.4 \\
        \bottomrule
    \end{tabular}
    \label{tab:semantics-aria}
\end{table}

% \begin{table}[ht]
%     \centering
%     \small
%     \setlength{\tabcolsep}{3pt}
%     \caption{Semantic Segmentation Evaluation on Aria}
%     \begin{tabular}{@{}lccc|lccc@{}}
%         \toprule
%         \multicolumn{4}{c|}{Sequences} & \multicolumn{4}{c}{Category} \\
%         \cmidrule(lr){1-4} \cmidrule(lr){5-8}
%         Scene & mIoU & fmIoU & mAcc & Class & mIoU & fmIoU & mAcc \\
%         \midrule
%         seq102  & 1.9 & 5.8 & 4.6 & head & 5.1 & 7.1 & 12.5 \\
%         seq134  & 1.8 & 7.0 & 4.7 & common & 0.1 & 0.1 & 0.8 \\
%         seq133  & 1.1 & 5.0 & 4.1 & tail & 0.0 & 0.0 & 0.2 \\
%          &  &  &  & overall & 1.7 & 6.5 & 4.4 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:semantics-aria}
% \end{table}

==> tables/slam-replica.tex <==
% \begin{table*}[ht]
%     \small
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{lcccccccc|c}
%         \toprule
%         & \multicolumn{8}{c}{Replica}\\
%         \cmidrule(lr){2-9}
%         \textbf{Method} 
%         & \rotatebox{90}{Room 0} 
%         & \rotatebox{90}{Room 1} 
%         & \rotatebox{90}{Room 2} 
%         & \rotatebox{90}{Office 0} 
%         & \rotatebox{90}{Office 1} 
%         & \rotatebox{90}{Office 2} 
%         & \rotatebox{90}{Office 3} 
%         & \rotatebox{90}{Office 4} 
%         & \rotatebox{90}{Freq. (Hz)}  \\
%         \midrule
%         CG-SLAM~\cite{CG-SLAM}  & 0.29 & 0.27 & 0.25 & 0.33 & 0.14 & 0.28 & 0.31 & 0.29 & 8.5  \\
%         SplaTAM~\cite{splatam}      & 0.31 & 0.40 & 0.29 & 0.47 & 0.27 & 0.29 & 0.32 & 0.55 & 0.21   \\
%         NICE-SLAM~\cite{NICE-SLAM}  & 0.97 & 1.31 & 1.07 & 0.88 & 1.00 & 1.06 & 1.10 & 1.13 & 0.98   \\
%         GS-ICP~\cite{GS-ICP-SLAM}  & 0.15 & 0.16 & 0.11 & 0.18 & 0.12 & 0.17 & 0.16 & 0.21 & 30   \\
%         GSORB~\cite{GSORB-SLAM}  & 0.35 & 0.22 & 0.33 & 0.33 & 0.19 & 0.54 & 0.63 & 0.45 & 1.61  \\
%         iMAP~\cite{iMAP}  & 3.12 & 2.54 & 2.31 & 1.69 & 1.03 & 3.99 & 4.05 & 1.93 & 10   \\
%         Co-SLAM~\cite{Co-SLAM}  & 0.65 & 1.13 & 1.43 & 0.55 & 0.53 & 0.46 & 1.49 & 0.77 & 14.2 \\
%         GO-SLAM~\cite{GO-SLAM}  & 0.32 & 0.30 & 0.39 & 0.39 & 0.46 & 0.34 & 0.29 & 0.29 & 8  \\
%         Loopy-SLAM~\cite{Loopy-SLAM}  & 0.24 & 0.24 & 0.28 & 0.26 & 0.4 & 0.29 & 0.22 & 0.35 &  0.1  \\
%         Point-SLAM~\cite{Point-SLAM}  & 0.61 & 0.41 & 0.37 & 0.38 & 0.48 & 0.54 & 0.72 & 0.63 & 0.48 \\
%         \textbf{Ours}               & - & - & - & - & - & - & - & -  & -  \\
%         \bottomrule
%     \end{tabular}
%     \caption{SLAM Performance Comparison on Replica and TUM-RGBD Dataset}
%     \begin{tablenotes}
%         \item Frequency evaluated on either Nvidia RTX 4090 or RTX 3090 GPU
%     \end{tablenotes}
%     \label{tab:slam-replica}
% \end{table*}

\begin{table}[t]
    \centering
    % \scriptsize
    \setlength{\tabcolsep}{1.2pt}
    \renewcommand{\arraystretch}{0.9}
    % \begin{threeparttable}
    \caption{SLAM Performance Comparison on Replica Dataset in cm (ATE)}
    \label{tab:slam-replica}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{lcccccccc|c}
            \toprule
            & \multicolumn{8}{c}{Replica}\\
            \cmidrule(lr){2-9}
            \textbf{Method} 
            & \rotatebox{90}{Room 0} 
            & \rotatebox{90}{Room 1} 
            & \rotatebox{90}{Room 2} 
            & \rotatebox{90}{Office 0} 
            & \rotatebox{90}{Office 1} 
            & \rotatebox{90}{Office 2} 
            & \rotatebox{90}{Office 3} 
            & \rotatebox{90}{Office 4} 
            & \rotatebox{90}{Average}  \\
            \midrule
            % CG-SLAM~\cite{CG-SLAM}      & 0.29 & 0.27 & 0.25 & 0.33 & 0.14 & 0.28 & 0.31 & 0.29 & 8.5  \\
            % SplaTAM~\cite{splatam}      & 0.31 & 0.40 & 0.29 & 0.47 & 0.27 & 0.29 & 0.32 & 0.55 & 0.21 \\
            % NICE-SLAM~\cite{NICE-SLAM}  & 0.97 & 1.31 & 1.07 & 0.88 & 1.00 & 1.06 & 1.10 & 1.13 & 0.98 \\
            % iMAP~\cite{iMAP}            & 3.12 & 2.54 & 2.31 & 1.69 & 1.03 & 3.99 & 4.05 & 1.93 & 10   \\
            % Co-SLAM~\cite{Co-SLAM}      & 0.65 & 1.13 & 1.43 & 0.55 & 0.53 & 0.46 & 1.49 & 0.77 & 14.2 \\
            % GO-SLAM~\cite{GO-SLAM}      & 0.32 & 0.30 & 0.39 & 0.39 & 0.46 & 0.34 & 0.29 & 0.29 & 8    \\
            VIPE~\cite{vipe}    & \textbf{2.40} & 3.75 & \textbf{3.92} & 6.37 & 14.49 & \textbf{6.05} & \textbf{1.89} & \textbf{1.88} & 5.09 \\
            KM-ViPE             & 3.80    & \textbf{1.66}    & 5.78    & 4.13    & 11.18    & 8.81    & 3.13    & 3.28    & 5.22    \\
            KM-ViPE$_{ark}$       & 3.25    & \textbf{1.66}    & 5.16    & \textbf{4.03}    & \textbf{10.30}    & 8.30    & 3.13    & 3.26   & \textbf{4.88}    \\
            \bottomrule
        \end{tabular}
    }%
    % \begin{tablenotes}
    % \end{tablenotes}
    % \end{threeparttable}
\end{table}


